RULER: What's the Real Context Size of Your Long-Context Language Models?

The needle-in-a-haystack (NIAH) test, which examines the ability to retrieve a piece of information (the "needle") from long distractor texts (the "haystack"), has been widely adopted to evaluate long-context language models (LMs). However, this simple retrieval-based test is indicative of only a superficial form of long-context understanding. To provide a more comprehensive evaluation of long-context LMs, we create a new synthetic benchmark RULER with flexible configurations for customized sequence length and task complexity. RULER expands upon the vanilla NIAH test to encompass variations with diverse types and quantities of needles. Moreover, RULER introduces new task categories multi-hop tracing and aggregation to test behaviors beyond searching from context. We evaluate 17 long-context LMs with 13 representative tasks in RULER. Despite achieving nearly perfect accuracy in the vanilla NIAH test, almost all models exhibit large performance drops as the context length increases. While these models all claim context sizes of 32K tokens or greater, only half of them can maintain satisfactory performance at the length of 32K. Our analysis of Yi-34B, which supports context length of 200K, reveals large room for improvement as we increase input length and task complexity. We open source RULER to spur comprehensive evaluation of long-context LMs.

==> Image/model_analysis_single.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.3\linewidth]{Image/pdf/Mamba.pdf}
    \includegraphics[width=0.3\linewidth]{Image/pdf/Mistral.pdf}
    \caption{TBD. \sscomment{contrast with mistralv2}}
    \label{fig:mamba-mistral}
\end{figure*}

==> Table/Deprecated/VT_example.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{p{0.1\linewidth}p{0.8\linewidth}}
    \toprule
        \multicolumn{2}{l}{\textbf{Generic Example of Variable Tracking (\textcolor{blue}{num\_chains=2}, \textcolor{blue}{num\_hops=2})}} \\ \midrule
        \textbf{Input:} & \textcolor{gray}{... (noises) ...} \textcolor{violet}{VAR X1 = 12345} \textcolor{gray}{......}  \textcolor{orange}{VAR Y2 = 54321} \textcolor{gray}{......} \textcolor{violet}{VAR X2 = VAR X1} \textcolor{gray}{......} \textcolor{orange}{VAR Y2 = VAR Y1}\textcolor{gray}{......} 
 \textcolor{violet}{VAR X3 = VAR X2}   
 \textcolor{gray}{......} 
 \textcolor{orange}{VAR Y2 = VAR Y1} \textcolor{gray}{......} \\
 \textbf{Query:} & Find all variables that are assigned the value 12345. \\
 \textbf{Target:} & \textcolor{violet}{X1 X2 X3}
 \\ 
         \bottomrule
    \end{tabular}
    \caption{Caption\sscomment{TODO: add new config row}}
    \label{tab:eg_vartrack}
\end{table}

==> Table/Deprecated/mamba_res.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}lccccc@{}}
\toprule
                               & 1k             & 2k    & 4k    & 8k  & 16k \\ \midrule
\textbf{noise k: words 1 v: numbers 1 r: 1} & 100.0 & 100.0 & 100.0 & 0.0 & 0.0 \\
\textbf{k: uuids $\infty$ v: uuids 1 r: 1}   & 4.6      & 0.0   & 0.0   & 0.0 & 0.0 \\
\textbf{book k: words 1 v: uuids 1 r: 1} & 100.0   & 99.4  & 0.2   & 0.0 & 0.0 \\
\textbf{variable\_tracking\_2\_2}    & 32.9   & 36.2  & 1.9   & 0.0 & 0.0 \\
\textbf{frequent word extraction alpha=3.5} & 81.5 & 81.9  & 54.5  & 1.0 & 0.0 \\ \bottomrule
\end{tabular}
\caption{Select task performance of Mamba-2.8B-slimpj. Mamba  }
\label{tab:mamba_result}
\end{table}


==> Table/res_ag.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|cc|cccccc|c|cc@{}}
\toprule
 \bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \begin{tabular}{@{}c@{}}\bf \small Effective\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(inc)\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(dec)\end{tabular}  \\

\midrule

Llama2-7B-chat & 4k & - & \multicolumn{4}{l}{84.8} & \\

\midrule

GPT-4 & 128k & 64k & \underline{99.0} & \underline{98.3} & \underline{98.0} & \underline{95.0} & \underline{90.1} & 79.7 & 93.4 & 90.4\rank{1st} & 96.3\rank{1st}  \\
Command-R (35B) & 128k & 16k & \underline{93.7} & \underline{93.8} & \underline{89.3} & 73.7 & 54.7 & 42.0 & 74.5 & 65.2\rank{4th} & 83.8\rank{2nd}  \\
Yi (34B) & 200k & 16k & \underline{91.4} & \underline{90.9} & \underline{86.2} & 75.3 & 58.5 & 43.4 & 74.3 & 66.0\rank{3rd} & 82.6\rank{3rd}  \\
Mixtral (8x7B) & 32k & 16k & \underline{91.7} & 82.7 & \underline{85.7} & 69.9 & 80.9 & 52.7 & 77.3 & 72.1\rank{2nd} & 82.4\rank{4th}  \\
Mistral (7B) & 32k & 8k & \underline{94.3} & \underline{90.4} & 77.4 & 48.5 & 42.4 & 33.7 & 64.4 & 53.1\rank{5th} & 75.8\rank{5th}  \\
ChatGLM (6B) & 128k & \textless{}4k & 79.6 & 64.3 & 53.5 & 43.2 & 39.6 & 35.5 & 52.6 & 45.4\rank{6th} & 59.9\rank{6th} \\
LWM (7B) & 1M & \textless{}4k & 61.3 & 43.6 & 38.3 & 32.8 & 29.1 & 29.1 & 39.0 & 34.0\rank{7th} & 44.0\rank{9th} \\
Together (7B) & 32k & \textless{}4k & 82.3 & 64.5 & 43.3 & 34.8 & 0.0 & 0.0 & 37.5 & 22.9\rank{9th} & 52.1\rank{7th} \\
LongChat (7B) & 32k & \textless{}4k & 74.3 & 50.7 & 46.7 & 51.1 & 0.0 & 0.0 & 37.1 & 24.8\rank{8th} & 49.5\rank{8th} \\
LongAlpaca (13B) & 32k & \textless{}4k & 33.0 & 27.0 & 26.0 & 23.2 & 0.0 & 0.0 & 18.2 & 12.3\rank{10th} & 24.1\rank{10th}  \\



\midrule\midrule

Llama2-7B (base) & 4k & - & \multicolumn{4}{l}{73.1} & \\

\midrule

Mixtral-base (8x7B) & 32k & 32k & \underline{96.5} & \underline{94.8} & \underline{93.1} & \underline{87.8} & 68.6 & 24.3 & 77.5 & 66.9\rank{1st} & 88.1\rank{1st}  \\
Mistral-base (7B) & 32k & 16k & \underline{94.8} & \underline{93.1} & \underline{81.6} & 53.3 & 36.7 & 9.2 & 61.4 & 46.5\rank{2nd} & 76.3\rank{2nd}  \\
Jamba-base (52B) & 256k & 4k & \underline{75.9} & 63.5 & 51.7 & 38.5 & 33.3 & 28.0 & 48.5 & 40.3\rank{3rd} & 56.6\rank{3rd}  \\
LWM-base (7B) & 1M & \textless{}4k & 67.1 & 48.4 & 36.0 & 26.3 & 21.5 & 18.7 & 36.3 & 28.4\rank{5th} & 44.2\rank{5th}  \\
LongLoRA-base (7B) & 100k & \textless{}4k & 70.3 & 64.4 & 50.7 & 39.9 & 29.4 & 0.0 & 42.4 & 31.3\rank{4th} & 53.6\rank{4th}  \\
Yarn-base (7B) & 128k & \textless{}4k & 70.6 & 49.2 & 28.9 & 20.5 & 17.0 & 2.1 & 31.4 & 20.7\rank{6th} & 42.0\rank{6th}  \\
Together-base (7B) & 32k & \textless{}4k & 69.1 & 53.0 & 19.9 & 20.6 & 0.0 & 0.0 & 27.1 & 15.1\rank{7th} & 39.1\rank{7th} \\


\bottomrule
\end{tabular}}
\vspace{-8pt}
\caption{Performance of selected aligned and base models across length 4k to 128k by averaging 2 task scores in Aggregation (CWE/FWE) of RULER.}
\label{tab:ag_result}
\end{table}


==> Table/res_main.tex <==
\begin{table}[t]
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{@{}l|cc|cccccc|c|cc@{}}
\toprule
 \bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \begin{tabular}{@{}c@{}}\bf \small Effective\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\\\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(inc)\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(dec)\end{tabular}  \\

\midrule

Llama2-7B (chat) & 4k & - & \multicolumn{4}{l}{85.6} & \\

\midrule

GPT-4 & 128k & 64k & \underline{96.6} & \underline{96.3} &  \underline{95.2} &  \underline{93.2} & \underline{87.0} & 81.2 & 91.6 & 89.0\rank{1st} & 94.1\rank{1st}  \\
Command-R (35B) & 128k & 32k &  \underline{93.8} &  \underline{93.3} &  \underline{92.4} & \underline{89.5} & 84.9 & 76.0 & 88.3 & 85.5\rank{2nd} & 91.1\rank{2nd}  \\
Yi (34B) & 200k & 32k &  \underline{93.3} &  \underline{92.2} &  \underline{91.3} & \underline{87.5} & 83.2 & 77.3 & 87.5 & 84.8\rank{3th} & 90.1\rank{3th}  \\
Mixtral (8x7B) & 32k & 32k &  \underline{94.9} &  \underline{92.1} &  \underline{92.5} & \underline{85.9} & 72.4 & 44.5 & 80.4 & 72.8\rank{4th} & 87.9\rank{4th}  \\
Mistral (7B) & 32k & 16k &  \underline{93.6} &  \underline{91.2} & \underline{87.2} & 75.4 & 49.0 & 13.8 & 68.4 & 55.6\rank{\textcolor{red}{7th}} & 81.2\rank{\textcolor{red}{5th}} \\
ChatGLM (6B) & 128k & 4k & \underline{87.8} & 83.4 & 78.6 & 69.9 & 56.0 & 42.0 & 69.6& 62.0\rank{6th} & 77.2\rank{6th} \\
LWM (7B) & 1M & \textless{}4k & 82.3 & 78.4 & 73.7 & 69.1 & 68.1 & 65.0 & 72.8 & 69.9\rank{\textcolor{red}{5th}} & 75.7\rank{\textcolor{red}{7th}}  \\
Together (7B) & 32k & 4k & \underline{88.2} & 81.1 & 69.4 & 63.0 & 0.0 & 0.0 & 50.3 & 33.8\rank{8th} & 66.7\rank{8th} \\
LongChat (7B) & 32k & \textless{}4k & 84.7 & 79.9 & 70.8 & 59.3 & 0.0 & 0.0 & 49.1 & 33.1\rank{9th} & 65.2\rank{9th} \\
LongAlpaca (13B)& 32k & \textless{}4k & 60.6 & 57.0 & 56.6 & 43.6 & 0.0 & 0.0 & 36.3 & 24.7\rank{10th} & 47.9\rank{10th} \\
\bottomrule
\end{tabular}}
\caption{Long Context Performance (\%) of selected models evaluated at length from 4k to 128k. Each score is computed by averaging  accuracy of 13 tasks in \ruler. The performance exceeding the Llama2-7B performance at 4K (85.6\%) is \underline{underlined}. The effective context  length is the maximum length passing this threshold. Weighted average score (wAvg.) aggregates performance across all context sizes, with the weights linearly increasing (inc) or decreasing (dec) to simulate length distribution of real-world usage. We put the rank of each model in the subscript. More details about the selected models are in Appendix~\ref{models}. }
\label{tab:main_result}
\end{table}

==> Table/res_mainv2.tex <==
\begin{table}[t]
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{@{}l|cc|cccccc|c|ll@{}}
\toprule
 \bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \begin{tabular}{@{}c@{}}\bf \small Effective\\\bf \small Length\end{tabular} & \bf4K & \bf8K & \bf16K & \bf32K & \bf64K & \bf128K & \begin{tabular}{@{}c@{}}\bf Avg.\\\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(inc)\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(dec)\end{tabular}  \\

\midrule

Llama2 (7B) & 4K & - & \multicolumn{4}{l}{85.6} & \\

\midrule

Gemini-1.5-pro & 1M & \textgreater{}128K & \underline{96.7} & \underline{95.8} &  \underline{96.0} &  \underline{95.9} & \underline{95.9} & \underline{94.4} & 95.8 & 95.5\rank{1st} & 96.1\rank{1st}  \\

GPT-4 & 128K & 64K & \underline{96.6} & \underline{96.3} &  \underline{95.2} &  \underline{93.2} & \underline{87.0} & 81.2 & 91.6 & 89.0\rank{2nd} & 94.1\rank{2nd}  \\

Qwen2 (72B) & 128K & 32K & \underline{96.9} & \underline{96.1} & \underline{94.9} & \underline{94.1} & 79.8 & 53.7 & 85.9 & 79.6\rank{\textcolor{red}{8th}} & 92.3\rank{\textcolor{red}{3rd}} \\

Command-R-plus (104B) & 128K & 32K &  \underline{95.6} &  \underline{95.2} &  \underline{94.2} & \underline{92.0} & 84.3 & 63.1 & 87.4 & 82.7\rank{\textcolor{red}{6th}} & 92.1\rank{\textcolor{red}{4th}}  \\

GLM4 (9B) & 1M & 64K & \underline{94.7} & \underline{92.8} & \underline{92.1} & \underline{89.9} & \underline{86.7} & 83.1 & 89.9 & 88.0\rank{\textcolor{red}{3rd}} & 91.7\rank{\textcolor{red}{5th}} \\

Command-R (35B) & 128K & 32K &  \underline{93.8} &  \underline{93.3} &  \underline{92.4} & \underline{89.5} & 84.9 & 76.0 & 88.3 & 85.5\rank{\textcolor{red}{4th}} & 91.1\rank{\textcolor{red}{6th}}  \\

GradientAI/Llama3 (70B) & 1M & 32K & \underline{95.1} & \underline{94.4} & \underline{90.8} & \underline{85.4} & 82.9 & 72.1 & 86.5 & 82.6\rank{7th} & 90.3\rank{7th} \\

Mixtral-8x22B (39B/141B) & 64K & 32K &  \underline{95.6} &  \underline{94.9} &  \underline{93.4} & \underline{90.9} & 84.7 & 31.7 & 81.9 & 73.5\rank{\textcolor{red}{11th}} & 90.3\rank{\textcolor{red}{8th}}  \\

Yi (34B) & 200K & 32K &  \underline{93.3} &  \underline{92.2} &  \underline{91.3} & \underline{87.5} & 83.2 & 77.3 & 87.5 & 84.8\rank{\textcolor{red}{5th}} & 90.1\rank{\textcolor{red}{9th}}  \\

Phi3-medium (14B) & 128K & 32K & \underline{93.3} & \underline{93.2} & \underline{91.1} & \underline{86.8} & 78.6 & 46.1 & 81.5 & 74.8\rank{10th} & 88.3\rank{10th} \\

Mixtral-8x7B (12.9B/46.7B) & 32K & 32K &  \underline{94.9} &  \underline{92.1} &  \underline{92.5} & \underline{85.9} & 72.4 & 44.5 & 80.4 & 72.8\rank{\textcolor{red}{12th}} & 87.9\rank{\textcolor{red}{11th}}  \\

GradientAI/Llama3 (8B) & 1M & 16K & \underline{92.8} & \underline{90.3} & \underline{85.7} & \underline{79.9} & 76.3 & 69.5 & 82.4 & 78.5\rank{\textcolor{red}{9th}} & 86.3\rank{\textcolor{red}{12th}} \\

Mistral (7B) & 32K & 16K &  \underline{93.6} &  \underline{91.2} & \underline{87.2} & 75.4 & 49.0 & 13.8 & 68.4 & 55.6\rank{\textcolor{red}{16th}} & 81.2\rank{\textcolor{red}{13th}} \\

GLM3 (6B) & 128K & 4K & \underline{87.8} & 83.4 & 78.6 & 69.9 & 56.0 & 42.0 & 69.6& 62.0\rank{\textcolor{red}{15th}} & 77.2\rank{\textcolor{red}{14th}} \\

LWM (7B) & 1M & \textless{}4K & 82.3 & 78.4 & 73.7 & 69.1 & 68.1 & 65.0 & 72.8 & 69.9\rank{\textcolor{red}{13th}} & 75.7\rank{\textcolor{red}{15th}}  \\

Phi3-mini (3.8B) & 128K & 4K &\underline{86.7} & 78.1 & 75.6 & 70.3 & 58.9 & 43.3 & 68.8 & 62.2\rank{\textcolor{red}{14th}} & 75.5\rank{\textcolor{red}{16h}} \\

DBRX (36B/132B) & 32K & 8K & \underline{95.1} & \underline{93.8} & 83.6 & 63.1 & 2.4 & 0.0 & 56.3 & 38.0\rank{17th} & 74.7\rank{17th} \\

Qwen1.5 (72B) & 32K & 8K & \underline{94.9} & \underline{93.8} & 78.0 & 67.8 & 0.0 & 0.0 & 55.7 & 37.5\rank{18th} & 74.0\rank{18th} \\

Together (7B) & 32K & 4K & \underline{88.2} & 81.1 & 69.4 & 63.0 & 0.0 & 0.0 & 50.3 & 33.8\rank{19th} & 66.7\rank{19th} \\

LongChat (7B) & 32K & \textless{}4K & 84.7 & 79.9 & 70.8 & 59.3 & 0.0 & 0.0 & 49.1 & 33.1\rank{20th} & 65.2\rank{20th} \\

LongAlpaca (13B)& 32K & \textless{}4K & 60.6 & 57.0 & 56.6 & 43.6 & 0.0 & 0.0 & 36.3 & 24.7\rank{21st} & 47.9\rank{21st} \\
\bottomrule
\end{tabular}}
\caption{Long Context Performance (\%) of selected models evaluated at length from 4K to 128K. Each score is computed by averaging  accuracy of 13 tasks in \ruler. The performance exceeding the Llama2-7B performance at 4K (85.6\%) is \underline{underlined}. The effective context  length is the maximum length passing this threshold. Weighted average score (wAvg.) aggregates performance across all context sizes, with the weights linearly increasing (inc) or decreasing (dec) to simulate length distribution of real-world usage. We put the rank of each model in the subscript. More details about the selected models are in Appendix~\ref{models}. }
\label{tab:main_result}
\vspace{-15pt}
\end{table}

==> Table/res_niah.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|cc|cccccc|c|cc@{}}
\toprule
 \bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \begin{tabular}{@{}c@{}}\bf \small Effective\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(inc)\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(dec)\end{tabular} \\

\midrule

Llama2-7B (chat) & 4k & - & \multicolumn{4}{l}{96.9} & \\

\midrule

GPT-4 & 128k & 32k & \underline{99.9} & \underline{99.9} & \underline{98.7} & \underline{98.3} & 90.9 & 84.8 & 95.4 & 92.9\rank{3rd} & 97.9\rank{2nd}  \\
Command-R (35B) & 128k & 64k & \underline{99.5} & \underline{99.3} & \underline{99.3} & \underline{98.9} &  \underline{97.4} & 89.6 & 97.3 & 96.0\rank{1st} & 98.6\rank{1st}  \\
Yi (34B) & 200k & 16k & \underline{98.1} & \underline{96.9} & \underline{97.4} & 95.1 & 93.0 & 90.2 & 95.1 & 93.8\rank{2nd} & 96.4\rank{3rd} \\
Mixtral (8x7B) & 32k & 16k & \underline{99.4} & \underline{98.3} & \underline{98.8} & 94.3 & 73.8 & 42.6  & 84.5 & 75.9\rank{5th} & 93.1\rank{4th}\\
Mistral (7B) & 32k & 4k & \underline{98.1} & 96.2 & 94.3 & 85.5 & 51.1 & 10.7 & 72.6 & 58.8\rank{7th} & 86.5\rank{7th}  \\
ChatGLM (6B) & 128k & 4k & \underline{97.5} & 95.9 & 91.9 & 83.6 & 67.6 & 50.9 & 81.2 & 73.5\rank{6th} & 89.0\rank{5th}  \\
LWM (7B) & 1M & \textless{}4k & 92.5 & 92.1 & 87.6 & 83.7 & 84.1 & 83.4 & 87.2 & 85.5\rank{4th} & 89.0\rank{6th} \\
Together (7B) & 32k & \textless{}4k & 96.2 & 89.9 & 82.3 & 80.2 & 0.0 & 0.0 & 58.1 & 40.2\rank{8th} & 76.0\rank{8th}  \\
LongChat (7B) & 32k & \textless{}4k & 93.3 & 92.2 & 81.1 & 67.3 & 0.0 & 0.0 & 55.7 & 37.6\rank{9th} & 73.7\rank{9th} \\
LongAlpaca (13B) & 32k & \textless{}4k & 74.9 & 72.2 & 70.8 & 53.2 & 0.0 & 0.0 & 45.2 & 30.7\rank{10th} & 59.7\rank{10th} \\



\midrule\midrule

Llama2-7B (base) & 4k & - & \multicolumn{4}{l}{90.9} & \\

\midrule

Mixtral-base (8x7B) & 32k & 32k & \underline{99.9} & \underline{99.7} & \underline{98.4} & \underline{94.8} & 72.1 & 29.1 & 82.3 & 71.8\rank{2nd} & 92.8\rank{1st} \\
Mistral-base (7B) & 32k & 16k & \underline{99.3} & \underline{97.5} & \underline{95.7} & 89.8 & 56.8 & 10.2 & 74.9 & 61.2\rank{4th} & 88.6\rank{2nd} \\
Jamba-base (52B) & 256k & \textless{}4k & 86.4 & 80.5 & 73.7 & 72.3 & 68.1 & 56.9 & 73.0 & 68.5\rank{3th} & 77.4\rank{5th}  \\
LWM-base (7B) & 1M & \textless{}4k & 88.5 & 87.7 & 84.5 & 79.6 & 76.1 & 74.2 & 81.8 & 79.1\rank{1st} & 84.4\rank{4th}  \\
LongLoRA-base (7B) & 100k & 16k & \underline{95.3} & \underline{95.6} & \underline{92.7} & 81.5 & 76.2 & 0.0 & 73.5 & 60.6\rank{5th} & 86.5\rank{3rd}  \\
Yarn-base (7B) & 128k & \textless{}4k & 89.9 & 86.1 & 78.4 & 59.0 & 49.5 & 17.5 & 63.4 & 51.7\rank{6th} & 75.1\rank{7th} \\
Together-base (7B) & 32k & 8k & \underline{95.4} & \underline{91.5} & 86.1 & 75.1 & 0.0 & 0.0 & 58.0 & 39.9\rank{7th} & 76.2\rank{6th} \\

\bottomrule
\end{tabular}}
\vspace{-8pt}
\caption{Performance of selected aligned and base models across length 4k to 128k by averaging 8 task scores in Retrieval (NIAH) of RULER.}
\vspace{-12pt}
\label{tab:niah_result}
\end{table}

==> Table/res_perfect.tex <==
\begin{table}[H]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|c|cccccc|c@{}}
\toprule

\bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\end{tabular} \\

\midrule

GPT-4 & 128k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Command-R (35B) & 128k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Yi (34B) & 200k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Mixtral (8x7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 97.0 & 99.5 \\
Mistral (7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 99.6 & 69.6 & 94.9 \\
ChatGLM (6B) & 128k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
LWM (7B) & 1M & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Together (7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 0.0 & 0.0 & 66.7 \\
LongChat (7B) & 32k & 100.0 & 100.0 & 100.0 & 99.4 & 0.0 & 0.0 & 66.6 \\
LongAlpaca (13B)& 32k & 88.2 & 88.6 & 86.4 & 82.4 & 0.0 & 0.0 & 57.6 \\


\midrule
\midrule

Mixtral-base (8x7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 46.8 & 91.1 \\
Mistral-base (7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 99.6 & 70.8 & 95.1 \\
Jamba-base (52B) & 256k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
LWM-base (7B) & 1M & 99.8 & 100.0 & 99.6 & 99.6 & 98.2 & 96.0 & 98.9 \\
LongLoRA-base (7B) & 100k & 99.6 & 99.4 & 99.0 & 99.4 & 99.4 & 0.0 & 82.8 \\
Yarn-base (7B) & 128k & 100.0 & 100.0 & 99.0 & 100.0 & 99.2 & 39.6 & 89.6 \\
Together-base (7B) & 32k & 100.0 & 100.0 & 99.8 & 100.0 & 0.0 & 0.0 & 66.6 \\

\bottomrule
\end{tabular}}
\caption{Performance of selected aligned and base models across length 4k to 128k in passkey retrieval of \ruler. Almost all models have perfect score at their claimed length.}
\label{tab:main_result_passkey}
\end{table}










\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|c|cccccc|c@{}}
\toprule

\bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\end{tabular} \\

\midrule

GPT-4 & 128k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Command-R (35B) & 128k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 98.0 & 99.7 \\
Yi (34B) & 200k & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Mixtral (8x7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 93.2 & 43.8 & 89.5 \\
Mistral (7B) & 32k & 100.0 & 100.0 & 100.0 & 97.0 & 70.0 & 7.4 & 79.1 \\
ChatGLM (6B) & 128k & 100.0 & 100.0 & 99.0 & 99.6 & 90.8 & 87.0 & 96.1 \\
LWM (7B) & 1M & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
Together (7B) & 32k & 100.0 & 100.0 & 100.0 & 99.8 & 0.0 & 0.0 & 66.7 \\
LongChat (7B) & 32k & 100.0 & 100.0 & 97.6 & 98.4 & 0.0 & 0.0 & 66.0 \\
LongAlpaca (13B) & 32k & 90.2 & 90.2 & 88.4 & 83.4 & 0.0 & 0.0 & 58.7 \\

\midrule
\midrule

Mixtral-base (8x7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 85.2 & 34.8 & 86.7 \\
Mistral-base (7B) & 32k & 100.0 & 100.0 & 100.0 & 100.0 & 94.8 & 0.4 & 82.5 \\
Jamba-base (52B) & 256k & 100.0 & 100.0 & 98.8 & 99.8 & 99.8 & 86.4 & 97.5 \\
LWM-base (7B) & 1M & 100.0 & 99.4 & 97.8 & 98.6 & 98.2 & 98.6 & 98.8 \\
LongLoRA-base (7B) & 100k & 99.8 & 100.0 & 100.0 & 99.8 & 100.0 & 0.0 & 83.3 \\
Yarn-base (7B) & 128k & 97.4 & 97.8 & 91.4 & 85.4 & 86.6 & 20.0 & 79.8 \\
Together-base (7B) & 32k & 100.0 & 100.0 & 100.0 & 99.8 & 0.0 & 0.0 & 66.6 \\

\bottomrule
\end{tabular}}
\caption{Performance of selected aligned and base models across length 4k to 128k in vanilla NIAH of \ruler. Almost all models have perfect score at their claimed length.}
\label{tab:main_result_passkey_2}
\end{table}

==> Table/res_qa.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|cc|cccccc|c|cc@{}}
\toprule
 \bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \begin{tabular}{@{}c@{}}\bf \small Effective\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(inc)\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(dec)\end{tabular} \\

\midrule

Llama2-7B (chat) & 4k & - & \multicolumn{4}{l}{49.7} & \\

\midrule

GPT-4 & 128k & 128k & \underline{79.0} & \underline{78.0} & \underline{76.0} & \underline{68.0} & \underline{61.6} & \underline{59.0} & 70.3 & 66.5\rank{1st} & 74.0\rank{1st}  \\
Command-R (34B) & 128k & 64k & \underline{67.9} & \underline{65.4} & \underline{63.9} & \underline{62.6} & \underline{58.1} & 48.4  & 61.1 & 58.2\rank{3rd} & 63.9\rank{4th}\\
Yi (34B) & 200k & 128k & \underline{72.7} & \underline{71.5} & \underline{68.4} & \underline{66.2} & \underline{64.1} & \underline{59.9}  & 67.1 & 65.0\rank{2nd} & 69.2\rank{2nd}\\
Mixtral (8x7B) & 32k & 64k & \underline{77.6} & \underline{73.0} & \underline{71.2} & \underline{64.5} & \underline{51.2} & 34.1  & 61.9 & 55.0\rank{5th} & 68.8\rank{3rd} \\
Mistral (7B) & 32k & 32k & \underline{72.4} & \underline{70.0} & \underline{65.7} & \underline{57.6} & 34.4 & 13.3 & 52.2 & 42.5\rank{6th} & 62.0\rank{5th} \\
ChatGLM (6B) & 128k & 16k & \underline{59.1} & \underline{53.5} & \underline{50.9} & 43.5 & 34.6 & 27.3 & 44.8 & 39.5\rank{7th} & 50.1\rank{7th}  \\
LWM (7B) & 1M & 128k & \underline{61.2} & \underline{57.8} & \underline{56.7} & \underline{55.4} & \underline{54.7} & \underline{52.6}  & 56.4 & 55.1\rank{4th} & 57.7\rank{6th} \\
Together (7B) & 32k & 16k & \underline{61.1} & \underline{58.3} & \underline{54.2} & 45.6 & 0.0 & 0.0 & 36.5 & 24.9\rank{8th} & 48.2\rank{8th} \\
LongChat (7B) & 32k & 8k & \underline{54.5} & \underline{53.6} & 47.6 & 34.0 & 0.0 & 0.0 & 31.6 & 21.0\rank{10th} & 42.3\rank{10th} \\
LongAlpaca (13B) & 32k & 16k & \underline{57.2} & \underline{53.5} & \underline{49.7} & 39.0 & 0.0 & 0.0 & 33.2 & 22.3\rank{9th} & 44.1\rank{9th} \\


\midrule\midrule

Llama2-7B (base) & 4k & - & \multicolumn{4}{l}{48.6} & \\

\midrule

Mixtral-base (8x7B) & 32k & 4k & \underline{50.8} & 47.7 & 45.3 & 41.3 & 34.4 & 26.4 & 41.0 & 37.0\rank{3rd} & 44.9\rank{3rd}  \\
Mistral-base (7B) & 32k & 8k & \underline{53.5} & \underline{51.0} & 48.4 & 44.7 & 32.8 & 2.2 & 38.8 & 31.3\rank{4th} & 46.3\rank{2nd}  \\
Jamba-base (52B) & 256k & 32k & \underline{62.7} & \underline{60.6} & \underline{57.9} & \underline{52.6} & 47.5 & 39.6 & 53.5 & 49.7\rank{1st} & 57.3\rank{1st}  \\
LWM-base (7B) & 1M & \textless{}4k & 42.7 & 40.2 & 38.7 & 37.1 & 37.3 & 34.6 & 38.4 & 37.2\rank{2nd} & 39.6\rank{4th}  \\
LongLoRA-base (7B) & 100k & \textless{}4k & 34.5 & 32.1 & 33.6 & 29.4 & 26.1 & 0.0 & 26.0 & 21.3\rank{6th} & 30.6\rank{6th}  \\
Yarn-base (7B) & 128k & \textless{}4k & 29.7 & 23.5 & 28.6 & 29.7 & 25.5 & 18.1 & 25.9 & 24.6\rank{5th} & 27.1\rank{7th}  \\
Together-base (7B) & 32k & 4k & \underline{52.0} & 47.5 & 44.6 & 33.6 & 0.0 & 0.0 & 29.6 & 19.8\rank{7th} & 39.5\rank{5th}  \\


\bottomrule
\end{tabular}}
\vspace{-8pt}
\caption{Performance of selected aligned and base models across length 4k to 128k by averaging 2 task scores in Question Answering of RULER.}
\label{tab:qa_result}
\end{table}

==> Table/res_vt.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|cc|cccccc|c|cc@{}}
\toprule
 \bf Models & \begin{tabular}{@{}c@{}}\bf \small Claimed\\\bf \small Length\end{tabular} & \begin{tabular}{@{}c@{}}\bf \small Effective\\\bf \small Length\end{tabular} & \bf4k & \bf8k & \bf16k & \bf32k & \bf64k & \bf128k & \begin{tabular}{@{}c@{}}\bf Avg.\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(inc)\end{tabular} & \begin{tabular}{@{}c@{}}\bf wAvg.\\\bf(dec)\end{tabular} \\

\midrule

Llama2-7B (chat) & 4k & - & \multicolumn{4}{l}{89.7} & \\

\midrule

GPT-4 & 128k & 128k & \underline{100.0} & \underline{100.0} & \underline{100.0} & \underline{100.0} & \underline{100.0} & \underline{99.6} & 99.9 & 99.9\rank{1st} & 100.0\rank{1st}  \\
Command-R (35B) & 128k & 128k & \underline{99.9} & \underline{100.0} & \underline{99.8} & \underline{99.5} & \underline{99.3} & \underline{89.8} & 98.1 & 96.8\rank{2nd} & 99.3\rank{2nd}  \\
Yi (34B) & 200k & 64k & \underline{99.8} & \underline{99.2} & \underline{98.8} & \underline{94.5} & \underline{92.5} & 76.8 & 93.6 & 90.3\rank{3rd} & 96.9\rank{3rd}  \\
Mixtral (8x7B) & 32k & 32k & \underline{99.9} & \underline{99.7} & \underline{98.4} & \underline{93.6} & 86.9 & 64.2 & 90.5 & 85.2\rank{4th} & 95.7\rank{4th}\\
Mistral (7B) & 32k & 16k & \underline{98.9} & \underline{96.0} & \underline{92.2} & 85.0 & 74.5 & 0.0  & 74.4 & 60.9\rank{5th} & 87.9\rank{5th}\\
ChatGLM (6B) & 128k & \textless{}4k & 84.0 & 81.2 & 78.0 & 66.0 & 38.4 & 13.0 & 60.1 & 48.3\rank{6th} & 71.9\rank{7th}  \\
LWM (7B) & 1M & \textless{}4k & 84.4 & 80.1 & 67.2 & 52.2 & 45.9 & 15.2 & 57.5 & 46.5\rank{7th} & 68.6\rank{8th} \\
Together (7B) & 32k & \textless{}4k & 89.2 & 88.8 & 48.3 & 16.6 & 0.0 & 0.0 & 40.5 & 22.8\rank{9th} & 58.2\rank{9th}  \\
LongChat (7B) & 32k & 8k & \underline{97.6} & \underline{93.5} & 83.4 & 62.4 & 0.0 & 0.0 & 56.2 & 37.4\rank{8th} & 75.0\rank{6th} \\
LongAlpaca (13B) & 32k & \textless{}4k & 8.5 & 2.1 & 18.2 & 17.0 & 0.0 & 0.0 & \ 7.6 & \ 6.5\rank{10th} & \ 8.8\rank{10th} \\



\midrule\midrule

Llama2-7B (base) & 4k & - & \multicolumn{4}{l}{58.8} & \\

\midrule

Mixtral-base (8x7B) & 32k & 64k & \underline{100.0} & \underline{99.9} & \underline{100.0} & \underline{98.4} & \underline{87.3} & 43.3 & 88.1 & 80.5\rank{2nd} & 95.8\rank{1st}  \\
Mistral-base (7B) & 32k & 64k & \underline{99.0} & \underline{98.4} & \underline{96.5} & \underline{89.1} & \underline{86.1} & 0.0 & 78.2 & 65.4\rank{4th} & 91.0\rank{2nd}  \\
Jamba-base (52B) & 256k & 128k & \underline{87.5} & \underline{87.6} & \underline{86.2} & \underline{88.1} & \underline{86.0} & \underline{77.8} & 85.5 & 84.3\rank{1st} & 86.7\rank{3rd}  \\
LWM-base (7B) & 1M & 128k & \underline{80.2} & \underline{82.7} & \underline{79.3} & \underline{76.4} & \underline{70.7} & \underline{66.1} & 75.9 & 73.3\rank{3th} & 78.5\rank{4th} \\
LongLoRA-base (7B) & 100k & 64k & \underline{92.5} & \underline{87.4} & \underline{73.1} & 56.0 & \underline{69.2} & 0.0 & 63.0 & 50.3\rank{5th} & 75.8\rank{5th} \\
Yarn-base (7B) & 128k & 4k & \underline{84.6} & 43.6 & 24.8 & 43.0 & 20.9 & 0.0 & 36.1 & 24.9\rank{7th} & 47.4\rank{7th} \\
Together-base (7B) & 32k & 16k & \underline{95.0} & \underline{90.6} & \underline{69.6} & 43.2 & 0.0 & 0.0 & 49.7 & 31.3\rank{6th} & 68.1\rank{6th}  \\


\bottomrule
\end{tabular}}
\vspace{-8pt}
\caption{Performance of selected aligned and base models across length 4k to 128k in Multi-hop tracing (VT) of RULER.}
\label{tab:vt_result}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
